Exploration Through Reward Biasing: Reward-Biased Maximum Likelihood Estimation for Stochastic Multi-Armed Bandits

Inspired by the Reward-Biased Maximum Likelihood Estimate method of adaptive control, we propose RBMLE -- a novel family of learning algorithms for stochastic multi-armed bandits (SMABs). For a broad range of SMABs including both the parametric Exponential Family as well as the non-parametric sub-Gaussian/Exponential family, we show that RBMLE yields an index policy. To choose the bias-growth rate $\alpha(t)$ in RBMLE, we reveal the nontrivial interplay between $\alpha(t)$ and the regret bound that generally applies in both the Exponential Family as well as the sub-Gaussian/Exponential family bandits. To quantify the finite-time performance, we prove that RBMLE attains order-optimality by adaptively estimating the unknown constants in the expression of $\alpha(t)$ for Gaussian and sub-Gaussian bandits. Extensive experiments demonstrate that the proposed RBMLE achieves empirical regret performance competitive with the state-of-the-art methods, while being more computationally efficient and scalable in comparison to the best-performing ones among them.

==> backup.tex <==
% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}{.5\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=18em]{figures/ID=16_Mean_T=3e5_Different_o(t).png}
%         \caption{Regret under different choices of $\alpha(t)$}
%         \label{fig:ID=16_Mean_T=3e5_Different_o(t)}
%     \end{subfigure}%
%     \begin{subfigure}{.5\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=18em]{figures/ID=16_Mean_T=3e5_Baselines.png}
%         \caption{Comparison of BMLE ($\alpha(t)=(\log(t))^{1.5}$) with state-of-the-art baselines}
%         \label{fig:ID=16_Mean_T=3e5_Baselines}
%     \end{subfigure}
%     \caption{Average cumulative regret of Gaussian Bandits over 100 trials with 5 arms: $\{\mu_i\}_{i=1}^{5} = \{1, 1.5, 0.5, 1.8, 0.8\}$ and $\sigma = 1.5$}
%     \label{fig:ID=16_Mean_T=3e5}
% \end{figure}


% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}{.5\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=18em]{figures/ID=15_Mean_T=3e4_Different_o(t).png}
%         \caption{Bayesian regret under different choices of $\alpha(t)$}
%         \label{fig:ID=15_Mean_T=3e4_Different_o(t)}
%     \end{subfigure}%
%     \begin{subfigure}{.5\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=18em]{figures/ID=15_Mean_T=3e4_Baselines.png}
%         \caption{Comparison of BMLE ($\alpha(t)=(\log(t))^{2}$) with state-of-the-art baselines}
%         \label{fig:ID=15_Mean_T=3e4_Baselines}
%     \end{subfigure}
%     \caption{Bayesian regret of Bernoulli Bandits over 80 instances with 10 arms: the parameter of each arm is drawn randomly from uniform distribution over $(0,1)$}
%     \label{fig:ID=15_Mean_T=3e4}
% \end{figure}


% \begin{figure}[H]
%     \centering
%     \begin{subfigure}{.39\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=13.5em]{figures/ID=5_Mean_T=3e5_Different_o(t).png}
%         \caption{Regret under different choices of $\alpha(t)$}
%         \label{fig:ID=5_Mean_T=3e5_Different_o(t)}
%     \end{subfigure}%
%     \begin{subfigure}{.39\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=13.5em]{figures/ID=5_Mean_T=3e5_Baselines.png}
%         \caption{Comparison of BMLE ($\alpha(t)=\log(t)$) with state-of-the-art baselines}
%         \label{fig:ID=5_Mean_T=3e5_Baselines}
%     \end{subfigure}
%     \caption{Average cumulative regret of Gaussian Bandits over 100 trials with 4 arms: $\{\mu_i\}_{i=1}^{4} = \{1.8, 2, 1.5, 2.5\}$ and $\sigma = 0.6$}
%     \label{fig:ID=5_Mean_T=3e5}
% \end{figure}



% \begin{table}[H]
% \begin{center}
% {\small
% \begin{tabular}{|p{2.4cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{2.3cm}|}
% \hline
% \textbf{Algorithm} & \textbf{BMLE} & \textbf{V-IDS} & \textbf{KG*} & \textbf{TS} & \textbf{UCB} & \textbf{GPUCB-Tuned}
% \\ \hline
% {\tt Mean Regret} & \textbf{\underline{0.82}} &  \textbf{\underline{0.78}} & 0.32 & 0.32 & 0.32 & 0.32
% \\ \hline
% {\tt Standard Error} & 0.77 & 0.75 & 0.27 & 0.32 & 0.32 & 0.32
% \\ \hline
% {\tt Quantile .10} & 0.66 & 0.38 & 0.26 & 0.32 & 0.32 & 0.32
% \\  \hline
% {\tt Quantile .25} & 0.59 & 0.28 & 0.32 & 0.32 & 0.32 & 0.32
% \\ \hline
% {\tt Quantile .50} & 0.75 & 0.31 & 0.32 & 0.32 & 0.32 &  \textbf{\underline{0.41}} 
% \\ \hline
% {\tt Quantile .75} & 0.61 & 0.78 & 0.18 & 0.18 & 0.18 & 0.18
% \\ \hline
% {\tt Quantile .90} & 0.61 & 0.78 & 0.18 & 0.18 & 0.18 & 0.18
% \\ \hline
% {\tt Quantile .95} & 0.61 & 0.78 & 0.18 & 0.18 & 0.18 & 0.18
% \\ \hline
% \end{tabular}
% }
% \end{center}

% \caption{Distribution statistics of final regret for Gaussian Bandits over 100 trials with 5 arms: $\{\mu_i\}_{i=1}^{5} = \{0.48, 0.49, 0.5, 0.51, 0.52\}$ and $\sigma = 0.8$}
% \end{table}\label{table:ID=18_Mean_T=3e5}



% \begin{figure}[H]
%     \centering
%     \begin{subfigure}{.39\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=13.5em]{figures/ID=3_Mean_T=3e4_Different_o(t).png}
%         \caption{Regret under different choices of $\alpha(t)$}
%         \label{fig:ID=3_Mean_T=3e4_Different_o(t)}
%     \end{subfigure}%
%     \begin{subfigure}{.39\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=13.5em]{figures/ID=3_Mean_T=3e4_Baselines.png}
%         \caption{Comparison of BMLE ($\alpha(t)=(\log(t))^{2}$) with state-of-the-art baselines}
%         \label{fig:ID=3_Mean_T=3e4_Baselines}
%     \end{subfigure}
%     \caption{Average cumulative regret of Bernoulli Bandits over 80 trials with true values: $\{\theta_i\}_{i=1}^{10}=\{0.76, 0.77, 0.78, 0.79, 0.8, 0.71, 0.72, 0.73, 0.74, 0.75\}$ }
%     \label{fig:ID=3_Mean_T=3e4}
% \end{figure}

% \vspace{-5mm}

% \begin{table}[H]
% \begin{center}
% {\small
% \begin{tabular}{|p{2.4cm}|p{1cm}|p{1cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{1cm}|p{0.6cm}|p{1cm}|}
% \hline
% \textbf{Algorithm} & \textbf{BMLE} & \textbf{V-IDS} & \textbf{IDS} & \textbf{KG*} & \textbf{KG} & \textbf{UCB} & \textbf{TUCB} & \textbf{TS} & \textbf{BUCB}
% \\ \hline
% {\tt Mean Regret} & \textbf{\underline{0.82}} &  \textbf{\underline{0.78}} & 0.32 & 0.32 & 0.32 & 0.32 & 0.32 & 0.32 & 0.32
% \\ \hline
% {\tt Standard Error} & 0.77 & 0.75 & 0.32 & 0.27 & 0.32 & 0.32 & 0.32 & 0.32 & 0.32
% \\ \hline
% {\tt Quantile .10} & 0.66 & 0.38 & 0.26 & 0.32 & 0.32 & 0.32 & 0.32 & 0.32 & 0.32
% \\  \hline
% {\tt Quantile .25} & 0.59 & 0.28 & 0.32 & 0.32 & 0.32 & 0.32 & 0.32 & 0.32 & 0.32
% \\ \hline
% {\tt Quantile .50} & 0.75 & 0.31 & 0.32 & 0.32 & 0.32 & 0.32 &  \textbf{\underline{0.41}} & 0.32 & 0.32
% \\ \hline
% {\tt Quantile .75} & 0.61 & 0.78 & 0.18 & 0.32 & 0.18 & 0.18 & 0.18 & 0.32 & 0.32
% \\ \hline
% {\tt Quantile .90} & 0.61 & 0.78 & 0.18 & 0.32 & 0.18 & 0.18 & 0.18 & 0.32 & 0.32
% \\ \hline
% {\tt Quantile .95} & 0.61 & 0.78 & 0.18 & 0.32 & 0.18 & 0.18 & 0.18 & 0.32 & 0.32
% \\ \hline
% \end{tabular}
% }
% \end{center}

% \caption{Distribution statistics of final regret (BUCB and TUCB refers to BayesUCB and UCB-Tuned as abbreviation) for Bernoulli Bandits over 80 trials with true values: $\{\theta_i\}_{i=1}^{10}=\{0.76, 0.77, 0.78, 0.79, 0.8, 0.71, 0.72, 0.73, 0.74, 0.75\}$}
% \end{table}\label{table:ID=3_Mean_T=3e4}
% \vspace{-8mm}



% \vspace{-5mm}
% \begin{figure}[H]
%     \centering
%     \begin{subfigure}{.39\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=13.5em]{figures/ID=5_Mean_T=3e5_Different_o(t).png}
%         \caption{Regret under different choices of $\alpha(t)$.}
%         \label{fig:ID=5_Mean_T=3e5_Different_o(t)}
%     \end{subfigure}%
%     \begin{subfigure}{.39\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=13.5em]{figures/ID=5_Mean_T=3e5_Baselines.png}
%         \caption{Comparison of BMLE ($\alpha(t)=\log(t)$) with state-of-the-art baselines.}
%         \label{fig:ID=5_Mean_T=3e5_Baselines}
%     \end{subfigure}
%     \caption{Average cumulative regret of Gaussian Bandits over 100 trials with 4 arms: $\{\mu_i\}_{i=1}^{4} = \{1.8, 2, 1.5, 2.5\}$ and $\sigma = 0.6$.}
%     \label{fig:ID=5_Mean_T=3e5}
% \end{figure}

% \subsection{Backup}
% \begin{figure}[H]
%     \centering
%     \begin{subfigure}{.39\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=13.5em]{figures/ID=3_Mean_T=3e4_Different_o(t).png}
%         \caption{Regret under different choices of $\alpha(t)$}
%         \label{fig:ID=3_Mean_T=3e4_Different_o(t)}
%     \end{subfigure}%
%     \begin{subfigure}{.39\textwidth}
%         \centering
%         \includegraphics[width=1\linewidth, , height=13.5em]{figures/ID=3_Mean_T=3e4_Baselines.png}
%         \caption{Comparison of BMLE ($\alpha(t)=(\log(t))^{2}$) with state-of-the-art baselines}
%         \label{fig:ID=3_Mean_T=3e4_Baselines}
%     \end{subfigure}
%     \caption{Average cumulative regret of Bernoulli Bandits over 80 trials with true values: $\{\theta_i\}_{i=1}^{10}=\{0.76, 0.77, 0.78, 0.79, 0.8, 0.71, 0.72, 0.73, 0.74, 0.75\}$ }
%     \label{fig:ID=3_Mean_T=3e4}
% \end{figure}




Moreover, since RBMLE directly operates with the likelihood function to guide the exploration instead of asking help from the concentration inequalities in proof, it may end up with quite different indices as illustrated by Table \ref{tab:my-table}\footnote{The fact that such qualitatively different indices provide excellent performance may be of interest but is not the scope of this paper.}. This makes it more challenging to quantify its finite-time performance. 
\begin{table}[!htbp]
\caption{Comparison of the RBMLE indices with indices from some UCB-family. Below, $H(p)$ is the binary entropy, $\overline{V}_{t}(i)$ is the upper bound on the variance, and the other quantities are defined in Sections \ref{section:formulation} and \ref{section:exponential}.}
\label{tab:my-table}
\begin{tabular}{|c|l|}
\hline
Algorithm             & \multicolumn{1}{c|}{Index}                                                      \\ \hline
\multirow{3}{*}{RBMLE} & (Bernoulli) $N_i(t)\big( H(p_i(t))-H(\tilde{p}_i(t)\big)$                       \\ \cline{2-2} 
                      & (Gaussian) $p_i(t)+\alpha(t)/(2N_i(t))$                                         \\ \cline{2-2} 
                      & (Exponential) $N_i(t)\log\big(\frac{N_i(t)p_i(t)}{N_i(t)p_i(t)+\alpha(t)}\big)$ \\ \hline
UCB                   & $p_i(t)+\sqrt{{2\log t}/{N_i(t)}}$                                          \\ \hline
UCB-Tuned             & $p_i(t) + \sqrt{\min\{\frac{1}{4}, \overline{V}_{t}(i)\}\log(t)/N_i(t)\}}$      \\ \hline
MOSS                  & $p_i(t)+\sqrt{\max(\log(\frac{T}{N_i(t)\cdot N}),0)/N_i(t)}$                    \\ \hline
\end{tabular}
\end{table}

In Bernoulli bandits, the reward of an arm $i$ is binary and drawn independently from a Bernoulli distribution with an unknown parameter $\theta_i \in (0, 1)$. In the setting of Gaussian bandits, the reward distribution of arm $i$ is a Gaussian distribution with mean $\mu_i$ and the standard deviation $\sigma_i$. For ease of presentation and to use the results of Proposition~\ref{prop:regret Gaussian}, we take $\sigma_i \equiv \sigma$ for all $i$ and assume knowledge of $\sigma$ in the experiments with Gaussian bandits. In exponential bandits, the reward distribution of arm $i$ follows an exponential distribution with the rate $\lambda_i$. 



It needs to be emphasized here that in Gaussian bandits, we choose the parameter values to make the problem very challenging: the standard deviation is 100 times the value difference between the largest mean and second-largest mean. We provide comparison under more randomly picked examples in Appendix~\ref{appendix:more empirical results}.

\section{Detailed Description of the Major Competitors}
\label{appendix:competitors}
The competitors from the frequentist setting include UCB~\cite{auer2002finite}, UCB-Tuned (UCBT)~\cite{auer2002finite}, MOSS~\cite{audibert2009minimax,degenne2016anytime}, and KL-UCB~\cite{garivier2011kl}.
On the other hand, the competitors from Bayesian family consist of Knowledge Gradient (KG)~\cite{ryzhov2012knowledge}, its variant - KG*~\cite{ryzhov2010robustness}, and the approximation KG* - KG(min) (KGMin), and MN (KGMN)~\cite{kaminski2015refined} in~\cite{kaminski2015refined}), Thompson sampling (TS)~\cite{chapelle2011empirical,kaufmann2012thompson,honda2014optimality}, Bayes-UCB (BUCB)~\cite{kaufmann2012bayesian}, Information Directed Sampling (IDS) and its variant - variance-based IDS (VIDS)~\cite{russo2014learning,russo2017learning}, and GPUCB~\cite{srinivas2012information} and its tuned version - GPUCB-Tuned (GPUCBT). GPUCB and GPUCBT are only regarded as competitors of BMLE in Gaussian bandits.

\subsection{Frequentist Approaches}
\label{appendix:freq}
The UCB algorithm selects an arm $i$ which maximizes the index $\widehat{\theta}_i(t) + \sqrt{2\log(t)/N_i(t)}$, where $\widehat{\theta}_i(t)$ is the empirical mean reward received from samples of arm $i$. The index of UCB is constructed to facilitate regret bound analysis. Its empirical performance is often unsatisfactory. To achieve better empirical performance, UCB-Tuned (UCBT) replaces the index by $\widehat{\theta}_i(t) + \sqrt{\min\{1/4, \overline{V}_{t}(i)\}\log(t)/N_i(t)\}}$, where $\overline{V}_{t}(i)$ is the upper bound on the variance of the reward of arm $i$. UCBT often demonstrates outstanding empirical performance but unfortunately, there is limited literature illustrating any guarantee to its regret bound. The MOSS algorithm uses $p_i(t)+\sqrt{\max(\log(\frac{T}{N_i(t)\cdot N}),0)/N_i(t)}$, a slightly different index from UCB and UCBT for arm $i$, where the computation of the index requires additional knowledge of time horizon $T$. It automatically decreases the amount of exploration after an arm has already been pulled more than $T/N$ times. It has two limitations: (1) sub-optimality - it is only \emph{nearly} asymptotically optimal, and can be arbitrarily worse than UCB in some regimes, and (2) instability - the distribution of the its regret can be not well-behaved. KL-UCB currently is the most computationally heavy method in the frequentist family. Taking Bernoulli bandits as an example, the index for arm $i$ is obtained through solving an optimization problem $\max\{p \in [0, 1]: D(p_{i}(t), p)\leq (\log(t) + c\log(\log(t))/N_{i}(t)\}$. The optimization problem often relies on Newton's method or bisection search to be solved, except in Gaussian bandits, a closed-form index can be derived thanks to the good form of KL divergence for Gaussian distributions. KL-UCB often demonstrates better empirical performance than UCB as it constructs the upper confidence bound using Chernoff's inequality, a tighter one than as has been used in UCB. 

\subsection{Bayesian Approaches}
\label{appendix:bayes}
GPUCB and GPUCBT are only for Gaussian bandits. Under GPUCB, the index of arm $i$ at time $t$ is $\mu_{i}(t) + \sqrt{\beta_t}\sigma_{i}(t)$, where $\mu_{i}(t)$ and $\sigma_{i}(t)$ are the posterior mean and posterior standard deviation for arm $i$ and $\beta_t = 2\log(N t^{2}\pi^{2}/6\delta)$. They provide regret bounds that hold with probability at least $1-\delta$. As such, $\delta$ is often chosen to be a very small positive number close to zero~\cite{russo2017learning}. Its variant GPUCB-Tuned (GPUCBT) demonstrates better empirical performance and replaces the original $\beta_t$ by $\beta_t=c\log(t)$, where $c$ is a hyperparameter tuned for time horizon $T$. Similar to UCBT, there is also concern about the theoretical guarantee on GPUCBT. Different from UCB-like algorithms, KG is inspired by the Bellman equation and is one type of the one-step look-ahead policy: the index for arm $i$ is determined by immediate reward of pulling arm $i$ and the expected future rewards after observing the outcomes of the pull. The future rewards are quantified by the knowledge improvement of the optimal arm after observing the outcome of the pulled arm in the current round. To be more specific, KG uses the index $\mu_i(t) + \mathbb{E}[\mu_*(t+1)-\mu_*(t)|i]$ for arm $i$, where $\mu_*(t) = \max_{i}\{\mu_i(t)\}$. KG has a closed form in both Bernoulli and Gaussian bandits. However, beyond limitations such as requiring time horizon $T$, the regret of KG sometimes grows linearly as it may explore insufficiently, especially when the outcome of true distribution is discrete and time horizon is long~\cite{kaminski2015refined}. To overcome this limitation, KG* was proposed by extending the one-step look-ahead to multi-step look-ahead. At time $t$, KG* calculates the index for an arm over all possible steps of look-ahead and thus suffer high computational complexity, which has very poor scaling performance with time horizon $T$. To enable longer time horizon evaluation, the heuristic approximation methods KGMin and KGMN were applied~\cite{kaminski2015refined}. Basically, they use
golden section search to maximize a non-concave function in the approximation, but are still empirically effective as illustrated in~\cite{russo2017learning}. TS in general works well for different types of bandits including those with discrete and continuous outcomes. It often outperforms vanilla UCB algorithms and follows a simple intuition: select the arm following the probability that it is the optimal arm. In each round, TS uses the outcome drawn from the posterior distribution of arm $i$ as its index for arm $i$. Motivated by Bayesian interpretation of the problem and to retain the simplicity of UCB-like algorithms in implementation, BUCB constructs upper confidence bounds based on the $1-1/t$ quantiles of posterior distribution. Specially, BUCB uses $Q_{i}\Big(1-1/\big(t(\log(T))^{c}\big)\Big)$ as the index for amr $i$, where $Q_{i}\big(\cdot\big)$ denotes the quantile function of the posterior distribution for arm $i$. Like MOSS and GPUCBT, BUCB also requires knowledge of time horizon $T$. TS and BUCB are proved to be optimal and observed to exhibit excellent performance in experiments with Bernoulli bandits. Their leading positions in empirical performance were displaced by IDS and its variant VIDS. In each round, IDS calculates the probabilities of pulling individual arms through solving an optimization problem $\min_{\bm{\pi}}\{\Delta_{t}^{2}(\bm{\pi})/g_{t}(\bm{\pi})\}$, where $\bm{\pi}$ is a vector of probabilities and $\bm{\pi}(i)$ denotes the probability of pulling arm $i$. $\Delta_{t}(\bm{\pi})$ denotes the expected regret under $\bm{\pi}$ and reward randomness. $g_{t}(\bm{\pi})$ denotes the entropy reduction with respect to the optimal arm. The exact computation of $\bm{\pi}$ and $g_{t}(\bm{\pi})$ requires computation of {multi-dimensional} integrals, which is very expensive. Therefore, usually sample-based estimation is applied. VIDS further approximates IDS through approximating $g_{t}(\bm{\pi})$ by $\bm{\pi}^{\top}\bm{v}$, where $\bm{v}$ denotes the vector of variance for all arms.



In the comparisons, the values of hyper-parameters are determined as follows. In IDS and VIDS, we sampled 100 points over $[0,1]$ interval for $q$ (Algorithm 4 in~\cite{russo2017learning}) and $M=10000$ (Algorithm 3 in~\cite{russo2017learning}). We take $c=0$ in BUCB and KL-UCB, which are reported to achieve the best empirical performance in the original papers. We take $c=0.9$ in GPUCBT after parameter tuning as in~\cite{russo2017learning}. In searching for a solution of KL-UCB and computing the value of $C_{\alpha,0}$, the maximum number of iterations is set to be 100. It is also worth mentioning that KL-UCB has the same closed-form index as UCB in Gaussian bandits. The conjugate priors for the approaches in the Bayesian family are Beta distribution $\beta(1,1)$ for Bernoulli bandits, $\mathcal{N}(0, 1)$ for Gaussian bandits, and Gamma distribution $\gamma(1,1)$ for exponential bandits. Most competitors are compared in all three types of reward distributions.

In Figure~\ref{fig:regret all 2} and Figure~\ref{fig:regret all 3}, we note that KG performs poorly as it explores insufficiently. This is not surprising as several papers have pointed out the limitations of KG, when rewards are discrete or the time horizon is long~\cite{kaminski2015refined}. When the rewards are continuous (e.g. in Gaussian bandits and exponential bandits), KG* and the variants of KG* (KGMin, KGMN) achieve remarkable performance improvement over the vanilla KG. This benefits from the consideration of more than one step in look-ahead planning. It is worth emphasizing that BMLE, in general, outperforms all other baselines, including IDS, VIDS and KL-UCB in terms of regret performance in all three types of bandits. It is not surprising that VIDS or IDS are the closest competitors to BMLE in terms of regret performance. However, BMLE is found to be slightly better than IDS and VIDS in those examples. Moreover, in spite of the good performance of IDS and VIDS, the determination of their indices suffers from high computational complexity, even under sample-based approximation. In contrast, the BMLE index, with its simple closed-form expression is trivial to compute. One more advantage of BMLE over some of the baselines is that it is ``time horizon agnostic'', i.e., the computation of BMLE index does not rely on the knowledge of time horizon $T$. In contrast, BUCB, MOSS, GPUCBT, and KG-family algorithms (KG, KG*) require the knowledge of $T$.


In Figure~\ref{fig:time all 2} and Figure~\ref{fig:time all 3}, the comparisons of efficiency of BMLE and other baseline methods are illustrated. Efficiency is represented by both metrics of interest: Computation time per decision as well as Regret. BMLE is seen to provide promising efficiency performance. Especially compared with IDS, VIDS, and KL-UCB, BMLE achieves slightly better regret performance with orders of magnitude less computation time per decision than those methods. IDS and VIDS suffer from high computation complexity because they need to estimate several integrals in each round. The KL-UCB often relies on Newton's method or bisection search to find the index for an arm, except in Gaussian bandits, where a closed-form solution can be obtained. We observe from the figure that those baselines such as UCB, GPUCB, and KG that also enjoy closed-form index have similar computation time per decision as BMLE, i.e., comparable vertical position in the Figure. However, their regret performance is far worse than BMLE's, i.e., larger horizontal position in the Figure, thus worse efficiency than BMLE. We also observe that in terms of efficiency, the closest competitors to BMLE are TS, MOSS and tuned version UCB (UCBT, GPUCBT). Compared to TS, BMLE follows the frequentist formulation and thus its performance does not deteriorate like TS when an inappropriate prior is mistakenly chosen. Compared to MOSS, BMLE does not rely on the knowledge of $T$ to compute its index. Compared to the tuned version UCB, the regret performance of BMLE enjoys stronger theoretical guarantees as illustrated by the aforementioned propositions.

\begin{comment}
\begin{table}[h]
\caption{Statistics of distribution of average final regret over 100 trials for the Gaussian bandits with true values: $\{\mu_i\}_{i=1}^{10}=\{0.46, 0.47, 0.48, 0.49, 0.5, 0.51, 0.52, 0.53, 0.54, 0.55\}$ and $T=10^{5}$ (We use GPUCBT and BUCB as the shorthand of GPUCB-Tuned and BayesUCB, respectively). }
\label{table:Gaussian_ID=11}
\begin{center}
{\small
%\begin{minipage}[b]{0.8\hsize}
\begin{tabular}{|p{2.4cm}|p{0.8cm}|p{0.8cm}|p{2.0cm}|p{1.0cm}|p{1.1cm}|p{0.7cm}|p{0.9cm}|p{0.8cm}|p{0.9cm}|}
\hline
\textbf{Algorithm} & \textbf{BMLE} & \textbf{VIDS} & \textbf{KLUCB\&UCB} & \textbf{GPUCB} & \textbf{GPUCBT} & \textbf{TS} & \textbf{BUCB} & \textbf{KG} & \textbf{KG*}  
\\ \hline
{\tt Mean Regret} & \textbf{\underline{860.0}} & 892.0 & 1885.1 & 2782.6 & 1191.7 & 773.9 & 1638.8 & 2247.2 & 1434.1
\\ \hline
{\tt Std. Error} & 792.0 & 682.7 & 258.1 & \textbf{\underline{182.7}} & 345.1 &	547.0 &	292.2 &	1917.2 & 379.4
\\ \hline
{\tt Quantile .10} & 125.0 & 297.9 & 1591.5 & 2529.6 & 764.5  & 240.1	& 1295.9 & \textbf{\underline{33.6}} & 1037.7
\\  \hline
{\tt Quantile .25} & \textbf{\underline{200.5}} & 440.4 & 1736.8 & 2664.4 & 1004.9 & 342.8 & 1398.3 & 1006.3 & 1195.9
\\ \hline
{\tt Quantile .50} & \textbf{\underline{413.4}} & 685.3 & 1887.0 & 2784.9 & 1158.6 & 511 & 1626.0 & 2017.6 & 1332.0
\\ \hline
{\tt Quantile .75} & \textbf{\underline{1207.0}} & 1227.3 & 2018.9 & 2908.0	& 1350.8 & 1260.7 & 1839.2 & 3991.6 & 1587.9
\\ \hline
{\tt Quantile .90} & 2126.4 & \textbf{\underline{1533.3}} & 2202.4 & 3016.2 & 1680.4 & 1539.0 & 2037.4 & 4085.9 & 2023.0
\\ \hline
{\tt Quantile .95} & 2319.3 & \textbf{\underline{2179.6}} & 2326.6	& 3069.3 & 1805.6 & 2001.0 & 2111.4 & 5095.5 & 2205.6
\\ \hline
\end{tabular}
%\end{minipage}
}
\end{center}
\end{table}
\end{comment}
